Data Management for Causal Algorithmic Fairness

Fairness is increasingly recognized as a critical component of machine learning systems. However, it is the underlying data on which these systems are trained that often reflects discrimination, suggesting a data management problem. In this paper, we first make a distinction between associational and causal definitions of fairness in the literature and argue that the concept of fairness requires causal reasoning. We then review existing works and identify future opportunities for applying data management techniques to causal algorithmic fairness.

==> Data Management For Algorithmic Fairness/macros.tex <==
%\usepackage{anysize}
%\usepackage{geometry}
%\geometry{top=1in, left=1in, right=1in, bottom=1in,footskip=.25in}
%\marginsize{1in}{0.8in}{1in}{1in}%tblr
%\usepackage[showframe,bottom=0.2in,footskip=.25in]{geometry}
%\usepackage[left=1in, right=1in, top=1in]{geometry}
%\newcommand{\cmt}[2]{\textcolor{dkmag}{[#1: #2]}}
%\newcommand{\personname}[1]{\cmt{Personname}{#1}}
%\newcommand{\standout}[1]{\textit{\textcolor{dkmag}{#1}}}
%usepackage[T1]{fontenc}
%\usepackage{fontspec}
%\setmainfont[Scale=0.85, Ligatures={Required,Common,Contextual,TeX}]{TeX Gyre Schola} % Incredible font inside latex

%
%\usepackage{fancyhdr}
%\usepackage{fullpage} %, hyperref}
%\usepackage{amssymb, amsmath, enumitem, titling, hyperref}
%\usepackage[standard]{ntheorem}
%%\usepackage[sort&compress]{natbib}
%\usepackage[top=0.65in, bottom=1.2in, left=0.95in, right=0.95in]{geometry}
% %\ifthenelse{\value{page}=1}
%          %{\setlength\headheight{40pt}}
%          %{\setlength\headheight{0pt}}
%
%\usepackage[backend=bibtex,sorting=anyt, maxnames=7, firstinits=true]{biblatex} %hyperref=true,
%\renewcommand*{\bibfont}{\footnotesize}
%\bibliography{bib_rs}
%%\renewcommand{\baselinestretch}{0.9}
\usepackage{multirow}
\usepackage{float}
\usepackage{caption}
%\usepackage{subfloat}
%\usepackage{float}
\usepackage{amsmath}
\usepackage{graphicx, multicol, latexsym, amsmath, amssymb}
\usepackage{blindtext}
\usepackage{caption}
\def\sharedaffiliation{%
\end{tabular}
\begin{tabular}{c}}
\newcommand{\vset}[1]{\mathbf{#1}}
%\usepackage{amsthm}
%
%\theoremstyle{definition}
%\newtheorem{definition}{Definition}[section]
% end Spencer

\newcommand{\reva}[1]{{ { { #1}}}}
\newcommand{\revb}[1]{{{ { #1}}}}
\newcommand{\revc}[1]{{{{ #1}}}}
\newcommand{\revd}[1]{{{{ #1}}}}
\newcommand{\reve}[1]{{{ { #1}}}}
%\newcommand{\revf}[1]{{{\color{red} {#1}}}}




\newcommand{\mypm}{\mathbin{\tikz [x=1.4ex,y=1.4ex,line width=.1ex] \draw (0.0,0) -- (1.0,0) (0.5,0.08) -- (0.5,0.92) (0.0,0.5) -- (1.0,0.5);}}%


\newcommand{\qii}{\delta}

\newcommand{\createcontingencytable}[4]{ %
	% #1=table name
	% #2=first column name
	% #3=new row sum name
	% #4=new column sum name
	\pgfplotstablecreatecol[
	create col/assign/.code={% In each row ...
		\def\rowsum{0}
		\pgfmathtruncatemacro\maxcolindex{\pgfplotstablecols-1}
		% ... loop over all columns, summing up the elements
		\pgfplotsforeachungrouped \col in {1,...,\maxcolindex}{
			\pgfmathsetmacro\rowsum{\rowsum+\thisrowno{\col}}
		}
		\pgfkeyslet{/pgfplots/table/create col/next content}\rowsum
	}
	]{#3}{#1}%
	%
	% Transpose the table, so we can repeat the summation step for the columns
	\pgfplotstabletranspose[colnames from={#2},input colnames to={#2}]{\intermediatetable}{#1}
	%
	% Sums for each column
	\pgfplotstablecreatecol[
	create col/assign/.code={%
		\def\colsum{0}
		\pgfmathtruncatemacro\maxcolindex{\pgfplotstablecols-1}
		\pgfplotsforeachungrouped \col in {1,...,\maxcolindex}{
			\pgfmathsetmacro\colsum{\colsum+\thisrowno{\col}}
		}
		\pgfkeyslet{/pgfplots/table/create col/next content}\colsum
	}
	]{#4}\intermediatetable
	%
	% Transpose back to the original form
	\pgfplotstabletranspose[colnames from=#2, input colnames to=#2]{\contingencytable}{\intermediatetable}
}
%

\PassOptionsToPackage{hyphens}{url}\usepackage{hyperref}
\newcommand{\inp}{{{\mb X }}}
\newcommand{\cm}{{{\mb M }}}
\newcommand{\acm}{{{\mb M_{\mc A} }}}
\newcommand{\cg}{ G}
\newcommand{\acg}{ G_{\mb M_{\mc A}} }

\newcommand{\nipsadult}{{{Binned Adult}}}
\newcommand{\nipscompas}{{{Binned COMPAS}}}
\usepackage{booktabs,siunitx}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
\newcommand{\fge}{{\bf {FGE}}}
\newcommand{\scmit}{{\bf {SNMIT}}}
\newcommand{\cmit}{{\bf {MIT}}}
\newcommand{\icmit}{{\bf {FNMIT}}}
\newcommand{\iscmit}{{\bf {FMIT}}}
\newcommand{\hcmit}{{\bf {HyMIT}}}
\newcommand{\ogsal}{{\bf {OGS}}}
\newcommand{\gsal}{{\bf {GS}}}
\newcommand{\pdal}{{\bf {CD}}}
\newcommand{\delay}{{\tt \textsc{Flight Delay}}}
\newcommand{\ate}{{\tt \textsc{ATE}}}
\newcommand{\nde}{{\tt \textsc{NDE}}}
\newcommand{\nie}{{\tt \textsc{NIE}}}
\newcommand{\E}{{\tt \mathbb{E}}}
\newcommand{\pr}{{\tt \mathrm{Pr}}}
\newcommand{\hsys}{{\textsc{HypDB}}}
\newcommand{\sys}{{\textsc{Capuchin}}}
\newcommand{\dal}{{{SGS}}}
\newcommand{\bigCI}{\mathrel{\text{\scalebox{1.07}{$\perp\mkern-10mu\perp$}}}}
\newcommand{\nbigCI}{\cancel{\mathrel{\text{\scalebox{1.07}{$\perp\mkern-10mu\perp$}}}}}
\newcommand{\rred}[1]{\textcolor{red}{#1}}
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\ind}[0]{\textrm{Indep}}
\newcommand{\ignore}[1]{}
\newcommand{\comlb}[1]{{\vspace{2mm}\noindent \rred{\bf COMM(Dan):}}~ #1 \hfill {\bf    END.}\\}
\newcommand{\combabak}[1]{{\vspace{4mm}\noindent \bf  COMM(Babak):}~ {\em \rred{#1}}\hfill {\bf END.}\\}



\newcommand*{\rom}[1]{\expandafter\@slowromancap\romannumeral #1@}

\newcommand{\dan}[1]{{{\color{red} {\bf\underline{Dan}}: [{#1}]}}}
\newcommand{\babak}[1]{{\texttt{\color{red} Babak: [{#1}]}}}
\newcommand{\bill}[1]{{\texttt{\color{olive} Bill: [{#1}]}}}
\newcommand{\luke}[1]{{\texttt{\color{blue} Luke: [{#1}]}}}
\newcommand{\johannes}[1]{{\texttt{\color{blue} Johannes: [{#1}]}}}
\newcommand{\red}[1]{{\textbf {{\color{red} [{#1}]}}}}
\newcommand{\scream}[1]{{\texttt{\color{red}{\textbf{[{#1}]}}}}}

\newcommand{\LOGSPACE}{{\scriptsize $  \mathrm{LOGSPACE}$}}
\newcommand{\NLOGSPACE}{{\scriptsize $  \mathrm{NLOGSPACE}$}}
\newcommand{\PTIME}{{\scriptsize $  \mathrm{PTIME}$ }}
\newcommand{\nindep}{\mbox{$\not\!\perp\!\!\!\perp$}}
\newcommand{\indep}{\mbox{$\perp\!\!\!\perp$}}





\newcommand{\tr}{1} %{\mathtt{t}}
\newcommand{\cn}{0} %{\mathtt{c}}

%infotheo
\newcommand{\rep}{D'}
\newcommand{\icq}{Q_\varphi}
\newcommand{\hb}{D^*}


\newcommand{\satt}{\mathbf{a}}
\newcommand{\att}{\mathbf{A}}
\newcommand{\sx}{\mathbf{x}}
\newcommand{\bx}{\mathbf{X}}
\newcommand{\pn}{\textmd{N}}
\newcommand{\ent}{{\mathcal{H}}}
\newcommand{\minf}{{{I}}}
\newcommand\mvd{\twoheadrightarrow}
\newcommand{\amvd}{\twoheadrightarrow_\alpha}
\newcommand{\fd}{\rightarrow}
\newcommand{\afd}{\rightarrow_\alpha}
\newcommand{\bfd}{\rightarrow_\beta}
\newcommand{\abfd}{\rightarrow_{\alpha+\beta}}
\newcommand{\A}{\texttt{A}}
\newcommand{\K}{\texttt{K}}
\newcommand{\deletelater}[1]{{\textbf {{\color{green} [{#1}]}}}}
\newcommand{\intervrel}{\texttt{intervened-relation}}

\newcommand{\annot}{\texttt{annot}}
\newcommand{\supp}{\texttt{supp}}
\newcommand{\sch}{{\mathcal{S}}}
\newcommand{\rel}{{\mathcal{R}}}
%\newcommand{\interv}{{\Gamma}}
\newcommand{\real}{{\mathbb{R}}}
\newcommand{\nat}{{\mathbb{N}}}
\newcommand{\explattr}{{\{E\}}}
%\newcommand{\change}{{\Delta}}
\newcommand{\bool}{{\textit{b}}}


\newcommand{\AP}{\texttt{AP}}
\newcommand{\highval}{\texttt{high}}
\newcommand{\midval}{\texttt{mid}}
\newcommand{\lowval}{\texttt{low}}
\newcommand{\aplow}{\texttt{poor}}
\newcommand{\aphigh}{\texttt{good}}
\newcommand{\dbnull}{\texttt{null}}
\newcommand{\relset}{\mathcal{R}}
\newcommand{\reltop}{{\mathcal{R}}_{top}}
\newcommand{\relbot}{{\mathcal{R}}_{bot}}
\newcommand{\attrset}{\mathcal{A}}
\newcommand{\attrtop}[1]{{\mathcal{A}}_{{top}, {#1}}}
\newcommand{\attrbot}{{\mathcal{A}}_{bot}}
%\newcommand{\featureset}{\mathcal{B}}
\newcommand{\wcl}{\mathscr{C}(\mb{C})}
\newcommand{\rwq}{{ {\mc{Q}_{rw}}}}
\newcommand{\db}{{D}}
\newcommand{\dbdom}{\mathbf{DB}}
\newcommand{\intervadditive}{{intervention-additive}}
\newcommand{\val}{{v}}
\newcommand{\valorig}{{u}}
%\newcommand{\dbdom}{\mathcal{D}}
\newcommand{\inputclass}{\mathcal{C}}
%\newcommand{\intervene}{\mathcal{I}}
%\newcommand{\tbaff}{{\tt{T_{Aff}}}}
%\newcommand{\attaff}{{\tt{A_{Aff}}}}
\newcommand{\univ}{{{U}}}
\newcommand{\pk}{{\mathtt{pk}}}
\newcommand{\fk}{{\mathtt{fk}}}
\newcommand{\expl}{{\phi}}
%\newcommand{\pk}{{\tt \mathtt{\pk}}}
\newcommand{\sign}{{\tt \mathtt{sign}}}
%\newcommand{\expldom}{{\Phi}}

\newcommand{\select}{\tt {\textsc{Select}}}
\newcommand{\where}{{\tt \textsc{Where}}}
\newcommand{\with}{{\tt \textsc{With}}}
\newcommand{\distinct}{{\tt \textsc{distinct}}}
\newcommand{\groupby}{{\tt \textsc{Group By}}}
\newcommand{\from}{{\tt \textsc{From}}}
\newcommand{\ct}{{\tt \textsc{Count}}}
\newcommand{\create}{{\tt \textsc{Create}}}
\newcommand{\explanation}{{\tt \textsc{Explanation}}}
%\newcommand{\Pr}{{\tt {Pr}}}
\newcommand{\on}{{\tt \textsc{On}}}
\newcommand{\sqlwith}{{\tt \textsc{With}}}
\newcommand{\as}{{\tt \textsc{as}}}
\newcommand{\cascade}{{\tt \textsc{Cascade}}}
\newcommand{\sqland}{{\tt \textsc{And}}}
\newcommand{\sqlin}{{\tt \textsc{In}}}
\newcommand{\true}{{\tt true}}
\newcommand{\false}{{\tt false}}
\newcommand{\inmath}[1]{{\mathtt {#1}}}

\newcommand{\RNum}[1]{\uppercase\expandafter{\romannumeral #1\relax}}
\newcommand{\ie}{{\em i.e.}} %\xspace}
\newcommand{\eg}{{\em e.g.}} %\xspace}
\newcommand{\etal}{{et al.}} %\xspace}
\newcommand{\aka}{{\em a.k.a.}\xspace}
\newcommand{\algorithmicbreak}{\textbf{Break}}
\newcommand{\backwd}{\mathcal{B}}
\newcommand{\mbl}{{\bf B}}
\newcommand{\mmb}{{\bf MB}}
\newcommand{\emb}{{ \bf MB}_\epsilon}
\newcommand{\embl}{{\bf B}_\epsilon}
\newcommand{\emmb}{{\bf IB}_{(\epsilon,\beta)}}
\newcounter{enumQues}
\newcommand{\mf}[1]{\mathrm{\mathfrak{#1}}}
\newcommand{\mb}[1]{{\mathbf{#1}}}
\newtheorem{defn}{Definition}[section]
\newtheorem{rem}[defn]{Remark}
\newtheorem{conj}[defn]{Conjecture}
\newtheorem{prop}[defn]{Proposition}
\newtheorem{obs}[defn]{Observation}
\newtheorem{assumption}[defn]{Assumption}
\newcommand{\proj}[1]{{\Pi}}
\newcommand{\sel}[1]{{\sigma}}

\newcommand{\un}[1]{{\underline{#1}}}
\newcommand{\ov}[1]{{\overline{#1}}}
\newcommand{\cut}[1]{}
\newcommand{\eat}[1]{}

\newcommand{\causalframework}{interventional fairness}
\newcommand{\metric}{interventional discrimination}
\newcommand{\fairalgorithm}{interventional fairness}

\newcommand{\defeq}{\stackrel{\text{def}}{=}}

\newcommand{\fairapp}{fairness application~}

